A Relational Intervention Approach for Unsupervised Dynamics Generalization in Model-Based Reinforcement Learning

The generalization of model-based reinforcement learning (MBRL) methods to environments with unseen transition dynamics is an important yet challenging problem. Existing methods try to extract environment-specified information $Z$ from past transition segments to make the dynamics prediction model generalizable to different dynamics. However, because environments are not labelled, the extracted information inevitably contains redundant information unrelated to the dynamics in transition segments and thus fails to maintain a crucial property of $Z$: $Z$ should be similar in the same environment and dissimilar in different ones. As a result, the learned dynamics prediction function will deviate from the true one, which undermines the generalization ability. To tackle this problem, we introduce an interventional prediction module to estimate the probability of two estimated $\hat{z}_i, \hat{z}_j$ belonging to the same environment. Furthermore, by utilizing the $Z$'s invariance within a single environment, a relational head is proposed to enforce the similarity between $\hat{{Z}}$ from the same environment. As a result, the redundant information will be reduced in $\hat{Z}$. We empirically show that $\hat{{Z}}$ estimated by our method enjoy less redundant information than previous methods, and such $\hat{{Z}}$ can significantly reduce dynamics prediction errors and improve the performance of model-based RL methods on zero-shot new environments with unseen dynamics. The codes of this method are available at \url{https://github.com/CR-Gjx/RIA}.

==> abstract.tex <==
% Although model-based reinforcement learning (RL) methods enjoy the benefits of high data efficiency and planning ability, they always fail to generalize well on new environments with unseen dynamics. 
% % their performance highly relies on the prediction accuracy of learned environmental dynamics, thus failing to generalize well on new tasks with unseen dynamics. 
% Existing methods try to incorporate context information into the dynamics prediction process to learn a generalized dynamics model robust to the change of environmental dynamics. However, contexts contain much redundant information unrelated to the dynamics change, leading to the spurious statistical association between the redundant information in contexts and dynamics, and thus harming the generalization ability. In this paper, we model the dynamics change as the difference of unobserved environment-specified factors $Z$ across environments. Because $Z$ is unobserved, how to specify $Z$ from contexts remains a big challenge. To tackle this problem, we propose two criteria that the estimated $\hat{Z}$ should satisfy but redundant information cannot: (a) The environment-specified factor $Z$ estimated from a single trajectory should be the same or similar because a trajectory samples from only one environment. (b) Given two same or semantically similar environment-specified factors, the outputs of the dynamics prediction model should be the same or similar if conditioned on the same state and action.
% According to the proposed criteria, we introduce a relational head to cluster factors $\hat{Z}$ estimated within the same trajectory. Then a counterfactual prediction module is proposed to find the $Z$ belong to the same environment but in different trajectories based on criteria (b). As a result, the redundant information in contexts that is conflict with the proposed criteria will be eliminated in estimated $\hat{Z}$, and thus improve the generalization ability of dynamics prediction model. 

% Model-based reinforcement learning (MBRL) methods enjoy the benefits of high data efficiency and planning ability, but they often fail to generalize well on new environments with unseen dynamics. 
% their performance highly relies on the prediction accuracy of learned environmental dynamics, thus failing to generalize well on new tasks with unseen dynamics. 
% Existing methods try to incorporate context information into the dynamics prediction process to learn a model robust to the change of environmental dynamics. However, the redundant information unrelated to the dynamics change in contexts will create a spurious statistical association with dynamics, undermining generalization ability. In this paper, we model the dynamics change as the variation of unobserved environment-specific factors $Z$ across environments. Because $Z$ is hidden, how to disentangle $Z$ from contexts remains a big challenge. To tackle this problem, we propose two criteria that the estimated $\hat{Z}$ should meet: (a) The environment-specific factor $Z$ estimated from a single trajectory should be the same because a trajectory is surely sampled from only one environment. (b) Given two semantically similar environment-specific factors, the outputs of the dynamics prediction model should be similar if conditioned on the same state and action.
% According to the proposed criteria (a), we introduce a relational head as a learnable function to enforce the similarity between two estimated $\hat{Z}$ from the same trajectory. Then, an interventional prediction module is proposed to find the $Z$ belonging to the same environment but in different trajectories based on criteria (b). As a result, the redundant information in contexts that conflicts with the proposed criteria will be eliminated in the estimated $\hat{Z}$, thus improving the generalization ability of the dynamics prediction model. 

%Generalizing Model-based reinforcement learning (MBRL) methods well in environments with unseen dynamics is a challenging and practical problem.
%Existing methods try to learn a  dynamics prediction model robust to the change of environmental dynamics by incorporating the context information $Z$ learned from past transition segments. However,  the redundant information unrelated to the dynamics change in transition segments will create a spurious statistical association with dynamics, undermining generalization ability.  In this paper, we model the dynamics change as the variation of unobserved environment-specified factors $Z$ across environments, but because $Z$ and environment labels are both unavailable, it is challenging to learn  $Z$ from transition segments without introducing redundant information. To tackle this problem, we introduce an interventional prediction module to find the $Z$ belonging to the same environment.
%Furthermore, by utilizing the $Z$'s invariance within a single environment, a relational head is proposed to maximize the mutual information between $\hat{{Z}}$ from the same environment. As a result, the redundant information in transition segments will be eliminated in the estimated $\hat{Z}$, thus improving the generalization ability of the dynamics prediction model. The experimental results on several benchmark datasets demonstrate that our approach can significantly reduce dynamics prediction errors and improve the performance of model-based RL methods on zero-shot new environments with unseen dynamics.

The generalization of model-based reinforcement learning (MBRL) methods to environments with unseen transition dynamics is an important yet challenging problem.
Existing methods try to extract environment-specified information $Z$ from past transition segments to make the dynamics prediction model generalizable to different dynamics. However, because environments are not labelled, the extracted information inevitably contains redundant information unrelated to the dynamics in transition segments and thus fails to maintain a crucial property of $Z$: $Z$ should be similar in the same environment and dissimilar in different ones. As a result, the learned dynamics prediction function will deviate from the true one, which undermines the generalization ability. To tackle this problem, we introduce an interventional prediction module to estimate the probability of two estimated $\hat{z}_i, \hat{z}_j$ belonging to the same environment.
Furthermore, by utilizing the $Z$'s invariance within a single environment, a relational head is proposed to enforce the similarity between $\hat{{Z}}$ from the same environment. As a result, the redundant information will be reduced in $\hat{Z}$. We empirically show that $\hat{{Z}}$ estimated by our method enjoy less redundant information than previous methods, and such $\hat{{Z}}$  can significantly reduce dynamics prediction errors and improve the performance of model-based RL methods on zero-shot new environments with unseen dynamics. The codes of this method are available at \url{https://github.com/CR-Gjx/RIA}.



%To tackle this problem, we propose two criteria that the estimated $\hat{Z}$ should meet: (a) The environment-specified factor $Z$ estimated from a single trajectory should be the same because a trajectory is surely sampled from only one environment. (b) Given two semantically similar environment-specified factors, the outputs of the dynamics prediction model should be similar if conditioned on the same state and action. According to the proposed criterion (a), we introduce a relational head as a learnable function to enforce the similarity between two estimated $\hat{Z}$ from the same trajectory. Then, an interventional prediction module is proposed to find the $Z$ belonging to the same environment but in different trajectories based on criterion (b). 


%Model-based reinforcement learning (MBRL) methods enjoy the benefits of high data efficiency and planning ability, but they often fail to generalize well on new environments with unseen dynamics. Existing methods try to incorporate context information learned from past transition segments into the dynamics prediction process to learn a model robust to the change of environmental dynamics. However, the redundant information unrelated to the dynamics change in transition segments will create a spurious statistical association with dynamics, undermining generalization ability. In this paper, we model the dynamics change as the variation of unobserved environment-specified factors $Z$ across environments. Because $Z$ is hidden, how to disentangle $Z$ from transition segments remains a big challenge. To tackle this problem, we propose two criteria that the estimated $\hat{Z}$ should meet: (a) The environment-specified factor $Z$ estimated from a single trajectory should be the same because a trajectory is surely sampled from only one environment. (b) Given two semantically similar environment-specified factors, the outputs of the dynamics prediction model should be similar if conditioned on the same state and action. According to the proposed criterion (a), we introduce a relational head as a learnable function to enforce the similarity between two estimated $\hat{Z}$ from the same trajectory. Then, an interventional prediction module is proposed to find the $Z$ belonging to the same environment but in different trajectories based on criterion (b). As a result, the redundant information in transition segments  that conflicts with the proposed criteria will be eliminated in the estimated $\hat{Z}$, thus improving the generalization ability of the dynamics prediction model. The experimental results on several benchmark datasets demonstrate that our approach can significantly reduce dynamics prediction errors and improve the performance of model-based RL methods on zero-shot new environments with unseen dynamics.

% (counterfactual)  Then we counterfactualy introduce a relational head cluster the estimated $Z$ across trajectories but show similar semantics.
% design a counterfactual relational approach to disentangle $Z$ from contexts. Firstly, we enforce the factor $\hat{Z}$ estimated
% we propose a counterfactual relational approach to estimate $Z$ in an unsupervised manner by utilizing intra-trajectory and inter-trajectory information to cluster $Z$ with similar semantics. Firstly,
% we propose a relational encoder to distil $Z$ from contexts into a latent vector and incorporate estimated $\hat{Z}$ into the dynamics prediction model as previous methods. Then taking advantage of the homogeneity of $Z$ in a single trajectory, we use a relational head to cluster factors within the same trajectory by the binary relation reasoning. Lastly, to cluster $Z$ from different trajectories but with similar semantics, 
% we introduce a counterfactual prediction module to measure the similarity between estimated $\hat{Z}$ from different trajectories. The similarity between factors will be assigned into relation head to infer multiply-relations of inter-trajectories, making the extracted factors $\hat{Z}$ more semantically meaningful. 
% The experimental results on several benchmark datasets demonstrate that our approach can significantly reduce dynamics prediction errors and improve the performance of model-based RL methods on zero-shot new environments with unseen dynamics.
 
% Lastly, we use a relational head to align the 
 
%%Lastly,  to measure how similarity of two $Z$ existing in different trajectories, we propose a counterfactual prediction module to calculate the prediction error of different $Z$ by
%Furthermore,   we introduce a conterfactual prediction module to the underlying 


%\textit{Unsupervised Dynamics generalization} aims to improve the robustness of model-based RL against the change of environmental dynamics, where the transition function $\mathcal{F}$ changes across training and test tasks, but $\mathcal{S}$, $\mathcal{A}$ and $\mathcal{R}$ remain the same.
% In this paper,
%We provide a new understanding of transition shift by modelling the shift as the change of unobserved confounders across different tasks. Furthermore, taking advantage of the homogeneity of the confounder in a trajectory, we propose a relational context encoder to extract the confounder information from the historical trajectory. The learned confounder vector enables both model-based reinforcement learning methods to be robust again transition shift and generalize well on tasks with unseen transition functions. 
%The experimental results on several benchmark datasets demonstrate the effectiveness of our method.

%Let $\mathcal{S}$ be the state space, $\mathcal{A}$ be the action space, $\mathcal{R}:\ \mathcal{S}\ \times  \mathcal{A} \rightarrow \mathbb{R}$ be the reward function, and $\mathcal{F}:\ \mathcal{S}\ \times  \mathcal{A} \rightarrow  \mathcal{S}$ be the transition function.  

==> conclusion.tex <==
In this paper, we propose a relational intervention approach to learn a generalized dynamics prediction model for dynamics generalization in model-based reinforcement learning.  Our approach models the dynamics change as the variation of environment-specified factor $\mathcal{Z}$ and explicitly estimates $\mathcal{Z}$ from past transition segments. Because environment label is not available, it is challenging to extract $\mathcal{Z}$ from transition segments without introducing additional redundant information.  We propose an intervention module to identify the probability of two estimated factors belonging to the same environment, and a relational head to cluster those  estimated $\hat{{Z}}$s  are from the same environments with high probability, thus reducing the redundant information unrelated to the environment. By incorporating the estimated  $\hat{{Z}}$ into the dynamics prediction process, the dynamics prediction model has a stronger generalization ability against the change of dynamics. The experiments demonstrate that our approach can significantly reduce the dynamics prediction error and improve the performance of model-based agents on new environments with unseen dynamics.
\newpage

==> discussion.tex <==
\subsection{Relation to Partially Observable Markov Decision Process (POMDP)}

\subsection{Relation to Offline Reinforcement Learning}

==> experiments.tex <==
In this section, we conduct experiment to evaluate the performance of our approach by answering the following questions: 
\begin{itemize}
	\item Can our approach reduce the dynamics prediction errors in model-based RL? (Section  \ref{sec:pred})
	\item Can our approach  promote the performance of model-based RL on environments with unseen dynamics? (Section  \ref{sec:per})
	\item Can our approach learn the semantic meaningful dynamics change? (Figuer \ref{fig:vis} and Appendix\ref{sec:vis})
	\item Is the similarity of $w$ measured by the intervention module reasonable? (Appendix  \ref{sec:wei})
	\item Can solely relational learning improve the performance of model-based RL? (Section  \ref{sec:aba})
\end{itemize}
\subsection{Enviromental Setup}
\textbf{Implementation Details} \quad Our approach includes three learnable functions, including relational encoder, relational head and prediction head. All three functions are constructed with MLP and optimized by Adam \citep{kingma2014adam} with the learning rate 1e-3. During the training procedure, the trajectory segments are randomly sampled from the same trajectory to break the temporal correlations of the training data, which was also adopted by \citep{seo2020trajectory,wang2020deep,wang2019dbsvec}. Specifically, the length of the transition segments, \emph{i.e.}, $k$, is 10. All implementation details can be found in Appendix \ref{sec:set}. \\\
\textbf{Datasets} \quad Following the previous methods \citep{lee2020context,seo2020trajectory}, we perform experiments on a classic control task (Pendulum) from OpenAI gym \citep{brockman2016openai} and simulated robotics control tasks (HalfCheetah, Cripple-HalfCheetah, Ant, Hopper, Slim-Humanoid) from Mujoco physics engine \citep{todorov2012mujoco}. \\
\textbf{Dynamics Settings} \quad  To change the dynamics of each environment, we follow previous methods \citep{zhou2019environment,packer2019assessing,lee2020context,seo2020trajectory} to change the environmental parameters (\emph{e.g.} length and mass of Pendulum) and predefine them in the training and test environmental parameters lists. At the training time, we randomly sample the parameters from the training parameter list to train our relational context encoder and dynamics prediction model. Then we test our model on the environments with unseen dynamics sampled from the test parameter list. Specifically,  the predefined parameters in the test parameter list are outside the training range. The predefined training and test parameter lists for each task are the same with \citep{lee2020context}, and all details are given in Appendix \ref{sec:set}. \\
\textbf{Planning} \quad  Following \citep{lee2020context,seo2020trajectory}, we use the model predictive model (MPC) \citep{maciejowski2002predictive} to select actions based on learned dynamics prediction model, and assume that the reward functions of environments are known.  Also, the cross-entropy method (CEM) \citep{de2005tutorial} is used to optimize action sequences for finding the best performing action sequences. \\
\textbf{Baselines} \quad  We compare our approach with following state-of-the-art model-based RL methods on dynamics generalization. Also, to show the performance gap between our method and supervised dynamics generalization, we perform the method using true environment label to cluster $Z$.
\begin{itemize}
	\item Probabilistic ensemble dynamics model (PETS) \citep{kurutach2018model}: PETS employs an probabilistic dynamics models to capture the uncertainty in modeling and planning. 
	\item Meta learning based model-based RL (ReBAL and GrBAL) \citep{nagabandi2018deep,nagabandi2018learning}: These methods train a dynamics model by optimizing a meta-objective \citep{finn2017model}, and update the model parameters by updating a hidden with a recurrent model  or by updating gradient updates at the test time.
	\item Context-aware dynamics model (CaDM) \citep{lee2020context}: This method design several auxiliary loss including backward and future states prediction to learn the context from transition segments.
	\item Trajectory-wise Multiple Choice Learning (TMCL) \citep{seo2020trajectory}: This method is the state-of-the-art model-based RL method on dynamics generalization, which introduces the multi-choice learning to cluster environments. {TMCL needs the adaptation in the test procedure, while our method does not, so we also report the performance of TMCL without adaptation in Figure \ref{exp:noadapt} for the fair comparison.} 
	\item True Label: The method uses our relational head to cluster $\hat{{Z}}$ with the true environment label (not the ground-truth of $Z$). All hyperparameters are same with our method for the fair comparison.
\end{itemize}

\subsection{Performance Comparisons with Baselines}
\subsubsection{Prediction Error Comparisons} \label{sec:pred}
We first evaluate whether the dynamics model trained by our methods can predict next-states more accurately or not.
Figure \ref{exp:pred} shows that the average dynamics prediction error of dynamics prediction models trained by three methods (CaDM \citep{lee2020context}, TMCL \citep{seo2020trajectory} and ours). We can see that the dynamics model trained by our relational intervention method has superior prediction performance over other state-of-the-art methods, achieving the lowest prediction errors on almost all six tasks. Specifically, the prediction errors of our model are lower than others by a large margin in Hopper and Pendulum, outperforming the state-of-the-art methods by approximately 10\%. 
\begin{figure}[!htb]
	%	\vspace{-1em}
	\vspace{-0.5em}
%%%	\begin{center}
%		\includegraphics[height=3.in]{figures/prediction.pdf}
		
%		\vspace{-0.5em}
%	\end{center}


		\centering
	
		\includegraphics[height=1.3in]{figures/prediction_iclr.pdf}
		%				             \includegraphics[width=1.2\textwidth]{MKDB_KDB_RMSE_ALL.pdf}
		%			\includegraphics[height=1.2in]{figures/training_aba.pdf}

%\label{exp:pred}
	\caption{{The average prediction errors of dynamics models on training environments during training process (over three times). Specifically, the x axis is the training timesteps and y axis is the $log$ value of average prediction prediction errors. More figures are given at Appendix \ref{sec:train}. } }
		\label{exp:pred}
%	\vspace{-0.5em}
		\vspace{-0.5em}
\end{figure}

\begin{table}[!htb]\centering 
	\setlength\tabcolsep{3pt}
	\small
	\vspace{-1em}
	\caption{The average rewards of baseline model-based RL methods and ours on test environments with unseen dynamics. Here we report the average rewards over three runs (ours is ten). Specifically, the results of methods with $*$ are from the paper \citep{lee2020context}.}
	\vspace{-0.3em}
	\begin{tabular}{cccccccc}
		\hline
		& PETS*  & ReBAL*                 & GrBAL*                 & CaDM                & TMCL & Ours & $\uparrow$ Ratio \\
		\hline
		Pendulum             & -1103   & -943.6  & -1137.9  & -713.95$\pm$21.1 &   -691.2$\pm$93.4   &  \textbf{-587.5}$\pm$64.4&15.0\%     \\
		
		Ant                  & 965.883.5  & 63.0& 44.7     & 1660$\pm$57.8    &   2994.9$\pm$243.8   &     \textbf{3297.9}$\pm$159.7 &10.1\%     \\
		Hopper               & 821.2& 846.2 & 621    & 845.2$\pm$20.41    &  999.35$\pm$22.8    &    \textbf{1057.4}$\pm$37.2&5.8\%   \\
		HalfCheetah          & 1720.9& 52 & -69.1   & 5876.6$\pm$799.0 &   9039.6$\pm$1065   &   \textbf{10859.2}$\pm$465.1&20.1\%  \\
		C\_HalfCheetah & 1572 & 868.7& 2814   & 3656.4$\pm$856.2 &   3998.8$\pm$856.2   &  \textbf{4819.3}$\pm$409.3 &20.5\% \\
		Slim\_Humanoid       & 784.5  & 97.25  & -480.7 & 859.1$\pm$24.01 &  2098.7$\pm$109.1     &   \textbf{2432.6}$\pm$465.1&15.9\% \\
		\hline
	\end{tabular}
	\vspace{-0.5em}
	\label{tab:perf}
\end{table}
\subsubsection{Performance Comparisons}\label{sec:per}
Then we evaluate the generalization of model-based RL agents trained by our methods and baselines on test environments with unseen dynamics. Following the setting of \citep{seo2020trajectory}, we perform experiments three runs (ours with 10 runs to reduce random errors), and give the mean of rewards at Table \ref{tab:perf}. We can see that the meta-learning based methods \citep{nagabandi2018deep,nagabandi2018learning}  do not perform better than vanilla PETS \citep{kurutach2018model}, while methods \citep{lee2020context,seo2020trajectory} that aim to learn a generalized dynamics prediction model are superior to others significantly. Among which our approach achieves the highest rewards on all six tasks among all methods. Figure \ref{exp:perf} shows the mean and standard deviation of average rewards during the training procedure, indicating that the performance of our methods is better than the other two methods consistently at the training time, which is sufficient to show the superiority of our method over other methods. {A fair comparison between TMCL (no adaptation) and our method can be found at Appendix \ref{sec:fair}}.
%In addition, Figure \ref{exp:perf} and Figure  \ref{exp:pred} show that the performance of model-based RL agents is highly correlated with the prediction error of trained dynamics function, \emph{e.g.} the lower prediction errors of our model in Hopper and Pendulum, and the higher performance of agents in these two tasks can be achieved. 
In addition, we observe that our method achieves comparable results with the method directly cluster $\hat{{Z}}$ using the truth environment label, which indicates that our intervention module actually can assign high similarities into  $\hat{{Z}}$s estimated from the same environment in an unsupervised manner. We also observe the same results in the similarity visualization in the Appendix \ref{sec:wei}, where we find that $\hat{{Z}}$s from the same environment are assigned significant higher similarities than those pairs from different environments. 
%However, although we have significantly lower prediction errors in Cripple\_Halfcheetah, the improvement on the agent's performance is marginal compared to other methods.  One possible reason is that the schemas of environmental-specified factors changing the dynamics function are different between training and test environments in the crippled setting. Thus, the prediction accuracy of the dynamics model decreases in the test environments, limiting the performance improvement. 

\begin{figure*}[!htb]
		
%	\begin{center}
\centering


				
				\includegraphics[height=1.3in]{figures/training_iclr.pdf}
			%				             \includegraphics[width=1.2\textwidth]{MKDB_KDB_RMSE_ALL.pdf}
%			\includegraphics[height=1.2in]{figures/training_aba.pdf}

%		\label{exp:perf}
		\vspace{-0.2em}
%	\end{center}
	\caption{{The average rewards of trained model-based RL agents on unseen test environments. The results show the mean and standard deviation of returns averaged over three runs. {The fair comparison between TMCL (no adaptation) and our method can be found in Appendix \ref{sec:fair}}} }
	\label{exp:perf}
		\vspace{-1em}
\end{figure*}


%
%\begin{table}[]\setlength{\tabcolsep}{1mm}
%	\begin{tabular}{lllllll}
%		\hline
%		& PETS               & ReBAL               & GrBAL               & CaDM                & TMCL & Ours \\
%		\hline
%		Pendulum             & -1103$\pm$47.7   & -943.6$\pm$95.9   & -1137.9$\pm$89.9  & -901.95$\pm$44.4  &      &      \\
%		
%		Ant                  & 965.8$\pm$85.0   & 63.0$\pm$16.4     & 44.7$\pm$5.2      & 1660$\pm$42.8     &      &      \\
%		Hopper               & 821.2$\pm$71.4   & 846.2$\pm$97.6    & 621$\pm$63.2      & 845$\pm$95.2      &      &      \\
%		HalfCheetah          & 1720.9$\pm$218.8 & 527$\pm$186.7  & -69.1$\pm$124.1    & 5876.6$\pm$1140.5 &      &      \\
%		C\_HalfCheetah & 1572$\pm$181.7   & 868.7$\pm$104.3 & 3.7$\pm$20        & 1956.4$\pm$431   &      &      \\
%		Slim\_Humanoid       & 784.5$\pm$446.1  & 97.25$\pm$373.2  & -480.7$\pm$215.3 & 859.1$\pm$309.35  &      &     \\
%		\hline
%	\end{tabular}
%\end{table}
%\subsubsection{Visulization}

\subsection{Ablation Study} \label{sec:aba}
%The Figure \ref{exp:aba} shows the
In this section, we evaluate the effect of the proposed relation head and intervention prediction on the generalization improvement, respectively.  Because the intervention prediction is based on the relational head, we compare the performance of our approach with and without the intervention. As Figure \ref{exp:aba_per} and \ref{exp:aba_pred} show, after incorporating the relational head and intervention prediction, the performance of model-based agents and the generalization of the dynamics prediction model are both improved. However, although the model without the intervention module has lower prediction errors in the Pendulum task, it also has lower rewards than the whole model. One possible reason is that the Pendulum is simple for the dynamics prediction model to learn, and thus the dynamics prediction model with the vanilla relational head is a little over-fitting on the training environments {(Please refer to prediction errors on test environments are given in Appendix \ref{sec:test})}, limiting the performance improvement. This phenomenon confirms the importance of our intervention prediction on reducing the trajectory-specified redundant information.
\begin{figure*}[!htb]
		\vspace{-0.5em}
%	\begin{center}
\centering
		\subfloat[]{      
			         \begin{minipage}[c]{.5\linewidth}
				             \centering
				             \label{exp:aba_per}
%				             \includegraphics[width=1.2\textwidth]{MKDB_KDB_RMSE_ALL.pdf}
				             \includegraphics[height=1.2in]{figures/training_aba.pdf}
				         \end{minipage}
			     }
		     \subfloat[]{         
			         \begin{minipage}[c]{.5\linewidth}
			             \centering
				             \includegraphics[height=1.2in]{figures/prediction_aba.pdf}
				              \label{exp:aba_pred}
				         \end{minipage}
			        
			     }
%		\includegraphics[height=1.2in]{figures/training_aba.pdf}
%		\includegraphics[height=1.2in]{figures/prediction_aba.pdf}
		
		\vspace{-0.8em}
%	\end{center}
	\caption{{(a) The average rewards of trained model-based RL agents on unseen environments. The results show the mean and standard deviation of returns averaged over three runs. (b) The average prediction errors over the training procedure. {Prediction errors on test environments are given in Appendix \ref{sec:test}}} }
		\vspace{-1.em}
\end{figure*}

==> intro_v2.tex <==
Reinforcement learning (RL) has shown great success in solving sequential decision-making problems, such as board games \citep{silver2016mastering, silver2017mastering, schrittwieser2020mastering}, computer games (\emph{e.g.} Atari, StarCraft II)  \citep{mnih2013playing, silver2018general, vinyals2019grandmaster}, and robotics \citep{levine2014learning, bousmalis2018using}. However, solving real-world problems with RL is still a challenging problem because the sample efficiency of RL is low while the data in many applications is limited or expensive to obtain \citep{gottesman2018evaluating, lu2018deconfounding, lu2020sample,kiran2020deep}.  Therefore, model-based reinforcement learning (MBRL) \citep{janner2019trust,kaiser2019model,schrittwieser2020mastering,zhang2019solar,van2019use,hafner2019learning,hafner2019dream,lenz2015deepmpc}, which explicitly builds a predictive model to generate samples for learning RL policy,  has been widely applied to a variety of limited data sequential decision-making problems.

However, the performance of MBRL methods highly relies on the prediction accuracy of the learned environmental model  \citep{janner2019trust}. Therefore, a slight change of environmental dynamics may cause a significant performance decline of MBRL methods \citep{lee2020context, nagabandi2018learning, seo2020trajectory}. The vulnerability of MBRL to the change of environmental dynamics makes them unreliable in real world applications. Taking the robotic control as an example \citep{nagabandi2018learning,yang2020data,rakelly2019efficient, gu2017deep,bousmalis2018using,raileanu2020fast,yang2019single}, dynamics change caused by parts damages could easily lead to the failure of MBRL algorithms.
% In addition, the dynamic changes of transition function in healthcare is 
%In the situation of absent data, a natural solution is to reuse the policy trained in similar tasks, \emph{e.g.} learning a policy in a simulator and adapt it into physical robotics with few additional training cost \citep{tobin2017domain}. Unfortunately, RL methods tend to overfit to tasks that they are trained on, and thus generalize poorly to other tasks and even partially perturbable tasks. \citep{cobbe2019quantifying,witty2018measuring,farebrother2018generalization,juliani2019obstacle,kostrikov2020image,song2019observational,justesen2018illuminating, packer2019assessing}.
This problem is called the \textit{dynamics generalization} problem in MBRL, where the training environments and test environments share the same state  $\mathcal{S}$  and action space $\mathcal{A}$ but the transition dynamics between states  $p(s_{t+1}|s_t,a_t)$  varies across different environments. Following previous works \citep{petersen2018precision,gottesman2018evaluating}, we focus on the \textbf{unsupervised dynamics generalization} setting, \emph{i.e.} the id or label information of dynamics function in training MDPs is not available. This setting appears in a wide range of applications where the information of dynamics function is difficult to obtain. For example, in healthcare, patients may respond differently to the same treatment, \emph{i.e.}, $p(s_{t+1}|s_t,a_t)$ varies across patients. However, it is difficult to label which patients share similar dynamics.

% Taking healthcare as an example, AI doctor needs to gives a patient treatment suggestion (\emph{i.e.} action $a_t$)  according to the patient's symptoms (\emph{i.e.} state $s_t$) at timestep $t$. However, patients may show different responses to identical treatments  (\emph{i.e.} dynamics function $\mathcal{F}: P(s_{t+1}|s_t,a_t)$), and even one patient may show different response during different time intervals, which increases the cost to obtain the id information of dynamics function during collecting data \citep{petersen2018precision,gottesman2018evaluating}, and thus we can only assume that the dynamics function is invariant in a certain time interval or  trajectory \citep{lee2020context,seo2020trajectory}.
% Various methods have been proposed to improve the performance of model-based RL methods in \textit{dynamics generalization} setting, \citep{doshi2016hidden,zhang2020learning} explore to define the change of transition function by a hidden parameter given the id of transition function. However, it is difficult to collect data with known transition function id. Taking healthcare as an example, AI doctor needs to gives a patient treatment suggestion (\emph{i.e.} action $a_t$)  according to patient's symptoms (\emph{i.e.} state $s_t$) at timestep $t$. However, patients may show different responses to identical treatments  (\emph{i.e.} transition function $\mathcal{F}: P(s_{t+1}|s_t,a)$) , and even one patient may show different response during different time intervals, which increases the cost to know the id of transition function during collecting data. As such, we consider the unsupervised dynamics generalization setting.

%The essential reason is that there are other factors  
%Various methods have been proposed to improve the generalization of RL methods in different settings,  among which we consider the \textit{dynamics generalization}, where the training tasks and test tasks share the same state and action space while the dynamics between states varies in different tasks.  \textit{dynamics generalization} appears in a wide range of real-world problems. Taking the smart treatment in healthcare as an example, AI doctor need to gives the patient treatment suggestion (\emph{i.e.} action $a_t$)  according to patients' symptoms (\emph{i.e.} state $s_t$) at timestep $t$. Unfortunately, patients may show different responses to identical treatments  (\emph{i.e.} transition function $\mathcal{F}: P(s_{t+1}|s_t,a)$) while the AI doctor based on RL methods cannot generalizes well on a new patient, making the deployment of AI doctor in real-world unreliable \citep{petersen2018precision,gottesman2018evaluating}. Furthermore, the change of transition function caused by parts damage is very common in the practical application of robots while RL based control algorithms always fail to deal with such emergency \citep{rakelly2019efficient, gu2017deep,bousmalis2018using}.

% for the simple HalfCheetah simulation in Mujoco engine \citep{todorov2012mujoco}, the change of transition function caused by a small modification of body mass can degrade the performance of the trained agent.. 
%These examples urge us to develop a reliable and robust to \textit{dynamics generalization} RL method for the deployment into the complex and practical real world applications.
\begin{figure}[!htb]
	\vspace{-1.6em}
	\centering
	\subfloat[]{      
		\begin{minipage}[c]{.28\linewidth}
			\label{fig:diagram}
			
			\includegraphics[scale=0.28]{figures/diagram.pdf}  \end{minipage}}
	%	\hspace{0.1in}
	\subfloat[]{      \begin{minipage}[c]{.23\linewidth}
			\includegraphics[scale=0.23]{figures/pca_pendulum_cadm.pdf}
			\label{fig:vis_cadm}
	\end{minipage}}
	%	\hspace{1in}
	\subfloat[]{      \begin{minipage}[c]{.23\linewidth}
			\includegraphics[scale=0.23]{figures/pca_pendulum_tmcl.pdf}\end{minipage}}
	%\hspace{1in}
	\subfloat[]{      \begin{minipage}[c]{.23\linewidth}
			\includegraphics[scale=0.23]{figures/pca_pendulum_our.pdf}\end{minipage}}
	\vspace{-1em}
	\caption{(a) The illustration of why historical states and actions are encoded in environment-specified factor $Z$, (b)(c)(d) The PCA visualizations of estimated context (environmental-specific) vectors in \textbf{Pendulum} task, where the dots with different colors denote the context vector (after PCA) estimated from different environments. More visualization results are given at Appendix \ref{sec:vis}.}
	\label{fig:vis}
	\vspace{-0.5em}
\end{figure}
To build a generalized dynamics prediction function that can generalize to different transition dynamics,  the shift of the transition dynamics can be modelled as the change of unobserved factors across different environments, \emph{i.e.} there are hidden environment-specified factors $Z \in \mathcal{Z}$ which can affect the environmental dynamics.  This is analogous to the human intuition to understand the change of dynamics, \emph{e.g.} patients may show different responses to identical treatments because the differences of their gene sequences can affect how well they absorb drugs \citep{wilke2007identifying}. It is natural to assume that $Z$ is the same in a single environment but varies across different environments. As such, these unobserved environment-specified factors do not violate the nature of  MDP in a single environment, but their changes can affect the dynamics functions across environments. Therefore, the dynamics function $f: \mathcal{S} \times \mathcal{A} \rightarrow \mathcal{S}$ can naturally be augmented by incorporating $Z$  to be $f: \mathcal{S} \times \mathcal{A} \times \mathcal{Z} \rightarrow \mathcal{S}$ \citep{rakelly2019efficient,zhou2019environment,lee2020context,seo2020trajectory}. 

Learning the augmented dynamics function is difficult because the environment-specified factor $Z$ is unobservable. Previous methods \citep{rakelly2019efficient,zhou2019environment,lee2020context} try to extract information from historical transition segments and use it as a surrogate for $Z$ (Figure \ref{fig:diagram}) . However, in the unsupervised dynamics generalization setting, the extracted information from historical transition segments inevitably contains redundant information unrelated to the dynamics.  The redundant information would cause the surrogate for $Z$ to lose a crucial property that characterizes $Z$: $Z$ should be similar in the same environment and dissimilar in different environments. As shown in Figure \ref{fig:vis_cadm}, the environment-specified information $\hat{Z}$ learned by CaDM \citep{lee2020context} does not form clear clusters for different environments. Because the learned $\hat{Z}$ fails to represent environmental information, the learned dynamics function will deviate from the true one, which undermines the generalization ability. To alleviate this problem, TMCL \citep{seo2020trajectory} directly clusters the environments by introducing multiple prediction heads, \emph{i.e.} multiple prediction functions. However, 
% as shown in Figure \ref{fig:vis_cadm}, the learned $\hat{Z}$ of TMCL also does not have satisfactory cluster structures. In addition,
TMCL needs to choose the proper prediction head for each new environment, making it hard to be deployed into the scenario with consistently changing environments, \emph{e.g.} robots walk in the terrain which is constantly changing. 
{To avoid adaptation at the deployment time, we thus need to learn a single generalized prediction function $\hat{{f}}$. To ensure that $\hat{{f}}$ can learn modals of transition dynamics in different environments, we need to cluster $Z$ according to their belonging environments.}

\begin{comment}
Because $Z$ is hidden, we cannot estimate $Z$ directly but can learn its mapping $T(Z)$ from past transition segments \citep{rakelly2019efficient,zhou2019environment,lee2020context} as its estimation $\hat{{Z}}$, where $T$ is a learned mapping function. Because $Z$ is the same within an environment, and thus we expect the estimated $\hat{{Z}}$s be similar if they are from the same environment, and vice versa. If we learn such clustered $\hat{{Z}}$, the learned mapping function $T$ would be bijective without considering that different environments have the same transition dynamics, and thus we can learn a dynamics function $f \circ T^{-1}$ as $\hat{f}$. However,  the environment label is not available in the unsupervised setting, so the redundant information unrelated to the environment, \emph{e.g.} historical states and actions information, is easily encoded into learned $\hat{{Z}}$ without the appropriate constraint about environments (Please refer to the \ref{fig:diagram}). Therefore, the learned context variables $\hat{{Z}}$s from different environments are always entangled  
%and the transition segments are not only constructed by $Z$ but also historical states and actions (Please refer to the \ref{fig:diagram}), Therefore, the learned context variables $\hat{{Z}}$s from different environments are always entangled  
(refer to CaDM \citep{lee2020context} in Figure \ref{fig:vis_cadm}) because such redundant information can appear in different environments, \emph{e.g.} one state can appear any environment share the same state space $\mathcal{S}$. Once the learned $\hat{{Z}}=T(Z)$ are entangled, there will exists an infinite number the inverse mapping function $T^{-1}$. As such, it is hard to learn the true estimated dynamics function $f \circ T^{-1}$ that can reflect the modals of transition dynamics in different environments, thus resulting in the limited improvement for dynamics generalization. 
% Previous methods \citep{rakelly2019efficient,zhou2019environment,lee2020context} try to learn $\hat{{Z}}$ from past transition segments, and incorporate it  into the dynamics prediction model to learn $f$. However, as Figure \ref{fig:vis_cadm} shows, the learned context variables $\hat{{Z}}$s from different environments by these methods are always entangled, which means that there exists an infinite number the inverse mapping function $T^{-1}$. As such, it is hard to learn the true estimated dynamics function $f \circ T^{-1}$ that can reflect the modals of transition dynamics in different environments, thus resulting in the limited improvement for dynamics generalization. 

To avoid this problem, TMCL \citep{seo2020trajectory} directly clusters the environments by introducing multiple prediction heads, \emph{i.e.} multiple prediction functions. However, TMCL needs to choose the proper prediction head for each new environment, and thus such further adaptation makes TMCL hard to be deployed into the scenario with consistently changing environment, \emph{e.g.} robots walk in areas where the terrain is constantly changing. Learning a single generalized prediction function can avoid further adaptation when deploying it into the real world, but to ensure that $\hat{{f}}$ can learn modals of transition dynamics in different environments, we need to cluster $Z$ according to their belonging environment.
\end{comment}
%However, as Figure \ref{fig:diagram} shows, the transition segments are not only constructed by $Z$ but also historical states and actions, so the redundant information unrelated to the environment, \emph{e.g.} historical states and actions information, is easily encoded into learned $\hat{{Z}}$ without the approtiate constraint about environments. Therefore, the learned context variables $Z$s from different environments are always entangled  (refer to CaDM in Figure \ref{fig:vis_cadm}) because the encoded redundant information can appear in different environments , \emph{e.g.} one state can appear any environment share the same state space $\mathcal{S}$. As such, the dynamics function $f$ learned by such estimated $\hat{{Z}}$ with redundant information is hard to learn the modals of transition dynamics in different environments, thus resulting in the limited improvement for dynamics generalization. 

% \citep{seo2020trajectory} models the change of transition functions across different task as a multi-modal distribution, \emph{i.e.} there are  unobserved task-specified factors $\{z_i,...,z_n\} \in Z$ can affect the transition function.
%we model the shift of the transition function as the change of unobservable factors across different tasks. 


% Obviously, incorporating the unobserved task-specified factors into the dynamic prediction model can improve the prediction accuracy in different tasks. However, because factors $\mathcal{C}$ is not observed, we need to estimate it in an unsupervised manner. 
%

In this paper, we provide an explicit and interpretable description to learn $Z$ as a vector $\hat{{Z}}$ {(\emph{i.e.} the estimation of $Z$)} from the history transition segments. To cluster $\hat{{Z}}$ from the same environment, we introduce a relational head module as a learnable function to enforce the similarity between $\hat{{Z}}$s learned from the same environments. However, because environment label is not available, we can only cluster the $\hat{{Z}}$s from the same trajectory, so we then propose an interventional prediction module to identify the probability of a pair of $\hat{z}_i, \hat{z}_j$ belonging to the same environment through estimating $\hat{Z}$'s direct causal effect on next states prediction by do-calculus \citep{pearl2000causality}.  Because $Z$s from the same environment surely have the same causal effect, we can directly maximize the similarity of $\hat{Z}$s with the similar causal effect using the relational head, and thus can cluster $\hat{Z}$ according to the estimated environmental similarity and alleviate the redundant information that varies in an environment, \emph{e.g.} historical states and actions. In the experiments, we evaluate our method on a range of tasks in OpenAI gym \citep{brockman2016openai} and Mujoco \citep{todorov2012mujoco}, and empirically show that $\hat{{Z}}$ estimated by our method enjoy less redundant information than baselines. The experimental results show that our method significantly reduces the model prediction errors and outperforms the state-of-art model-based RL methods \textbf{without any adaptation step} on a new environment, and even achieve comparable results with the method directly cluster $\hat{{Z}}$ with the true environment label. 
%Specifically,  the average rewards of our methods are higher than those of TMCL \citep{seo2020trajectory} by 38\% in the classical HalfCheetah task. 


% summarize two criteria that the environment-specified factors $Z$ should meet, according to the nature of the dynamics generalization setting: (a) The environment-specified factors $Z$ estimated from a single trajectory should be the same, because a trajectory must be sampled from only one environment;  (b) According to the extended generalized dynamics function $f: \mathcal{S} \times \mathcal{A} \times \mathcal{Z} = \mathcal{S}$, if the state and action remain the same, the outputs of dynamics function should be similar given two semantically similar estimated $\hat{{Z}}$. 

%Based on the two criteria, we propose a relational intervention approach to estimate ${Z}$ from the trajectories.  Specifically, according to criterion (a), we introduce a relational head module as a learnable function to enforce the similarity between estimated $\hat{{Z}}$ from the same trajectory, which eliminates  transition segments-specified redundant information. However, only clustering $\hat{{Z}}$ in the same trajectory cannot remove the trajectory-specified redundant information without the environment id of each trajectory.

%To identify trajectories belonging to the same environment, 
% his is because different trajectories may be sampled from the same environment, and thus the factors $\hat{\mathcal{Z}}$ belonging to these trajectories can share the same or similar semantics. 
%we propose an interventional prediction module to measure the similarity between estimated $\hat{{Z}}$ from different trajectories based on the criterion (b), where we model the dynamics prediction model as a structural causal model and solely estimate the causal effect of $\hat{Z}$ on next states prediction by do-calculus \citep{pearl2000causality}.
% estimated $\hat{Z}$ will be concatenated with all state-action pairs in a mini-batch to predict next states. 
%According to the criterion (b) and the generalized dynamics function $f: \mathcal{S} \times \mathcal{A} \times \mathcal{Z} = \mathcal{S}$, high similarities will be assigned into factors $\hat{{Z}}$ that have similar prediction distributions. Similar as before, the proposed relational head module can impose similarity on the factors Z across trajectiries with similar semantics, and thus the estimated $\hat{{Z}}$ can generalize on different trajectories and eliminate the trajectory-specified spurious redundant information. In the experiments, we evaluate our method on a range of tasks in OpenAI gym \citep{brockman2016openai} and Mujoco \citep{todorov2012mujoco}, and the experimental results show that our method significantly reduce the model prediction errors and outperforms the state-of-art model-based RL methods. Specifically,  the average rewards of our methods are higher than those of TMCL \citep{seo2020trajectory} by 38\% in the classical HalfCheetah task. 
% two criteria, we propose a relational intervention approach to estimate unobserved environment-specified factors  $Z$ explicitly.
% and semantic meaningfully and improve the generalization ability of model-based RL. Firstly, we use an encoder to distil the unobserved task-specified factors $Z$  into a vector from transition segments of each task, and then the distilled vector $\hat{Z}$ is incorporated into the dynamics prediction model $f$ in the model-based RL methods, enabling the estimated $\hat{Z}$ can help $f$ generalize well on other tasks with unseen dynamics. Then taking advantage of the homogeneity of the $Z$ in a single trajectory, a relational head is used to discriminate whether the distilled factor vector relates to vectors from the same trajectory, which clusters the estimated $\hat{Z}$ from the same trajectory without modelling irrelevant dependencies, \emph{e.g.} context information. Lastly, we propose a interventional prediction module to make full use of inter-trajectory information in a mini-batch, making the learned task-specified factor  $\hat{Z}$ more semantically meaningful. This module infers the multiple-relations between task-specified factors $Z$ in different trajectories by measuring their similarities. Every estimated factor $\hat{z_i} \in \hat{Z}$  in a mini-batch will be used to predict the next state belong to other trajectories in this module, \emph{i.e.} interventional prediction. The high similarity will be assigned to those factors that have similar next state predictions over a mini-batch \emph{e.g.} two factors are from trajectories but belong to the same task. By means of relational head, we can cluster factors $\hat{Z}$ with similar semantics but in different trajectories in an unsupervised manner.
% In the experiments, we evaluate our method on a range of tasks in OpenAI gym \citep{brockman2016openai} and Mujoco \citep{todorov2012mujoco}, and the sufficient results show that the performance of our method exceeds the state-of-art model-based RL methods.


%\textbf{Contribution} (1) We propose a encoder based on the relational learning, enabling the 

% (distilled factors from the same trajectory) or not (with distilled factor from other trajectories). 

%of the distilled   and relational learning, the proposed encoder is trained to maximize the mutual information between trajectories and underlying confounder, and discard the useless information, \emph{e.g.} context information, thus disentangling meaningful confounder embedding from history trajectory.

%In the experiments, we combine the confounder embedding extracted from proposed contrastive confounder encoder into both model-based RL and model-free RL methods, and then evaluate them on a range of tasks in OpenAI gym \citep{brockman2016openai} and Mujoco \citep{todorov2012mujoco}. Sufficient experimental results show:
%\begin{enumerate}
%	\item Our contrastive confounder encoder shows superior generalization ability on unseen tasks with different transition functions, and the performance even exceed state-of-the-art RL methods.
%	\item Our contrastive confounder encoder shows higher sample-efficiency on model-based RL.
%	\item The visualization results
%\end{enumerate}
% the sights, scents, andsounds of baking, driven by a propose a confounder encoder to distill the confounder information that can potentially change the transition function.
%
%taking a tennis game as an example, when you 
%is so high that they need a large amount of data or interactions with the environment to optimize the agent's behaviour.  
% different opponents will hit back the tennis ball in different policies when facing the same incoming ball, and thus you need to 



%To learn the generalized dynamics function   $f: \mathcal{S} \times \mathcal{A} \times \mathcal{Z} \rightarrow \mathcal{S}$, our model provides an explicit and interpretable description to learn $Z$. Because environment labels are unavailable, we cannot directly cluster $Z$s estimated from the same environment and learn $Z$ as the environment invariant information. As such,  ${Z}$ estimated from the history transition segments inevitably contains the redundant information unrelated to environmental specific. To filter out such redundant information, we introduce a relational head module as a learnable function to maximize the mutual information between $\hat{{Z}}$s learned from the same environments. Still, because environment label is not available, we can only cluster the $Z$s from the same trajectory, but only cluster $Z$s from the same trajectory is not e
%so we then propose an interventional prediction module to identify trajectories belonging to the same environment through estimating the similarity of $\hat{Z}$'s causal effect on next states prediction by do-calculus \citep{pearl2000causality}.  Because the $Z$ from the same environment surely have the same causal effect on the By simultaneously updating relational head and maximize the similarity of $\hat{Z}$s with the similar causal effect, the environmental invariant information will be encoded into $\hat{{Z}}$, and thus eliminate the spurious redundant information within the transition segments and a single trajectory. In the experiments, we evaluate our method on a range of tasks in OpenAI gym \citep{brockman2016openai} and Mujoco \citep{todorov2012mujoco}, and the experimental results show that our method significantly reduces the model prediction errors and outperforms the state-of-art model-based RL methods. Specifically,  the average rewards of our methods are higher than those of TMCL \citep{seo2020trajectory} by 38\% in the classical HalfCheetah task. 

==> introduction.tex <==
Reinforcement learning (RL) has shown great success in sequential decision-making problems, such as boarding game (Go, Chess and Shogi) \cite{silver2016mastering, silver2017mastering, schrittwieser2020mastering}, computer games (\emph{e.g.} Atari, StarCraft II)  \cite{mnih2013playing, silver2018general, vinyals2019grandmaster}, and robotics \cite{levine2014learning, bousmalis2018using}. However, solving real-world problems with RL is still a challenging problem because the sample efficiency of RL is low while the data in many applications is limited or expensive, such as the treatment policy in healthcare \cite{gottesman2018evaluating, lu2018deconfounding, lu2020sample} and autonomous driving \cite{kiran2020deep}.  Therefore, model-based reinforcement learning (MBRL) approaches \cite{janner2019trust,kaiser2019model,schrittwieser2020mastering,zhang2019solar}, which explicitly build a predictive model to generate samples for training RL policy,  have been widely applied to a variety of limited data sequential decision-making problems because of their high data-efficiency.


However, the performance of MBRL methods highly relies on the prediction accuracy of the learned environmental model  \cite{janner2019trust,lai2020bidirectional}. Therefore, a slight change of environmental dynamics may cause a significant performance decline of MBRL methods \cite{lee2020context, nagabandi2018learning, seo2020trajectory}. The vulnerability of model-based RL against the change of environmental dynamics makes them unreliable when deploying into complex and changeable real-world applications. Taking the control of a robot as an example \cite{nagabandi2018learning,yang2020data,rakelly2019efficient, gu2017deep,bousmalis2018using}, parts damage is very common in the practical application of robots, which always results in the change of the dynamics of robots,  while model-based RL based control algorithms always fail to deal with such emergency, resulting in the accident and danger after deploying robots.
% In addition, the dynamic changes of transition function in healthcare is 

%In the situation of absent data, a natural solution is to reuse the policy trained in similar tasks, \emph{e.g.} learning a policy in a simulator and adapt it into physical robotics with few additional training cost \cite{tobin2017domain}. Unfortunately, RL methods tend to overfit to tasks that they are trained on, and thus generalize poorly to other tasks and even partially perturbable tasks. \cite{cobbe2019quantifying,witty2018measuring,farebrother2018generalization,juliani2019obstacle,kostrikov2020image,song2019observational,justesen2018illuminating, packer2019assessing}.


The above example can be summarized as  \textit{dynamics generalization} problem in the model-based reinforcement learning, where the training environments and test environments share the same state  $\mathcal{S}$  and action space $\mathcal{A}$ but the dynamics function between states  $\mathcal{F}: \mathcal{S} \times \mathcal{A} = \mathcal{S}$ varies in different environments. Here we focus on the unsupervised dynamics generalization, \emph{i.e.} the id or label information of dynamics function in training MDPs is not available. This setting appears in a wide range of applications where the information of dynamics function is difficult to obtain.
Taking healthcare as an example, AI doctor needs to gives a patient treatment suggestion (\emph{i.e.} action $a_t$)  according to the patient's symptoms (\emph{i.e.} state $s_t$) at timestep $t$. However, patients may show different responses to identical treatments  (\emph{i.e.} dynamics function $\mathcal{F}: P(s_{t+1}|s_t,a_t)$), and even one patient may show different response during different time intervals, which increases the cost to obtain the id information of dynamics function during collecting data \cite{petersen2018precision,gottesman2018evaluating}, and thus we can only assume that the dynamics function is invariant in a certain time interval or  trajectory \cite{lee2020context,seo2020trajectory}.
% Various methods have been proposed to improve the performance of model-based RL methods in \textit{dynamics generalization} setting, \cite{doshi2016hidden,zhang2020learning} explore to define the change of transition function by a hidden parameter given the id of transition function. However, it is difficult to collect data with known transition function id. Taking healthcare as an example, AI doctor needs to gives a patient treatment suggestion (\emph{i.e.} action $a_t$)  according to patient's symptoms (\emph{i.e.} state $s_t$) at timestep $t$. However, patients may show different responses to identical treatments  (\emph{i.e.} transition function $\mathcal{F}: P(s_{t+1}|s_t,a)$) , and even one patient may show different response during different time intervals, which increases the cost to know the id of transition function during collecting data. As such, we consider the unsupervised dynamics generalization setting.

%The essential reason is that there are other factors  
%Various methods have been proposed to improve the generalization of RL methods in different settings,  among which we consider the \textit{dynamics generalization}, where the training tasks and test tasks share the same state and action space while the dynamics between states varies in different tasks.  \textit{dynamics generalization} appears in a wide range of real-world problems. Taking the smart treatment in healthcare as an example, AI doctor need to gives the patient treatment suggestion (\emph{i.e.} action $a_t$)  according to patients' symptoms (\emph{i.e.} state $s_t$) at timestep $t$. Unfortunately, patients may show different responses to identical treatments  (\emph{i.e.} transition function $\mathcal{F}: P(s_{t+1}|s_t,a)$) while the AI doctor based on RL methods cannot generalizes well on a new patient, making the deployment of AI doctor in real-world unreliable \cite{petersen2018precision,gottesman2018evaluating}. Furthermore, the change of transition function caused by parts damage is very common in the practical application of robots while RL based control algorithms always fail to deal with such emergency \cite{rakelly2019efficient, gu2017deep,bousmalis2018using}.

% for the simple HalfCheetah simulation in Mujoco engine \cite{todorov2012mujoco}, the change of transition function caused by a small modification of body mass can degrade the performance of the trained agent.. 
%These examples urge us to develop a reliable and robust to \textit{dynamics generalization} RL method for the deployment into the complex and practical real world applications.

To improve the generalization of the dynamics model in model-based RL, previous methods \cite{rakelly2019efficient,zhou2019environment,lee2020context} try to incorporate the context variables or vectors into the dynamics prediction model. However, the contexts contains much redundant information unrelated to the dynamics change, and the dynamics prediction model will create spurious statistic association with redundant information, making the learned context variables from different environments are entangled (See Figure ) \cite{lee2020context}, resulting in the limited improvement for the dynamics generalization. 
Then \cite{seo2020trajectory}  introduces multi-choice learning and trajectory level information to cluster the trajectories implicitly, but it still remains unknown how to specify the dynamics change explicitly in an interpretable way.

% \cite{seo2020trajectory} models the change of transition functions across different task as a multi-modal distribution, \emph{i.e.} there are  unobserved task-specified factors $\{z_i,...,z_n\} \in Z$ can affect the transition function.
%we model the shift of the transition function as the change of unobservable factors across different tasks. 
In this paper, we model the shift of the dynamics function as the change of unobserved factors across different environments, \emph{i.e.} there are unobserved environment-specified factors $\{z_i,...,z_n\} \in \mathcal{Z}$ can affect the environmental dynamics.  This is analogous to the human intuition to understand the change of dynamics, \emph{e.g.} patients may show different responses to identical treatments because their underlying genetic difference can affect how well they absorb drugs \cite{wilke2007identifying}, different pole lengths also result in variations of dynamic functions in CartPole tasks. Specifically, $\mathcal{Z}$ is invariant in a single environment but varies in different environments. As such, these unobserved environment-specified factors do not violate the nature of  MDP in a single environment, but their changes can affect the dynamics functions across environments. Therefore, the dynamics function can be extended from $\mathcal{F}: \mathcal{S} \times \mathcal{A} = \mathcal{S}$  to   $\mathcal{F}: \mathcal{S} \times \mathcal{A} \times \mathcal{Z} = \mathcal{S}$ to generalize on different environments. 

% Obviously, incorporating the unobserved task-specified factors into the dynamic prediction model can improve the prediction accuracy in different tasks. However, because factors $\mathcal{C}$ is not observed, we need to estimate it in an unsupervised manner. 
%

However, because $\mathcal{Z}$ is hidden, how to disentangle $\mathcal{Z}$ from contexts remains a big challenge. We summary two criteria that the environment-specified factor $\mathcal{Z}$ should meet according to the nature of the dynamics generalization setting: (a) Because a trajectory is surely sampled from only one environment, the environment-specified factors $\mathcal{Z}$ estimated from a single trajectory should be the same. (b) According to the extended generalized dynamics function $\mathcal{F}: \mathcal{S} \times \mathcal{A} \times \mathcal{Z} = \mathcal{S}$, if the state and action remain the same, the outputs of dynamics function should be similar given two semantically similar estimated $\hat{\mathcal{Z}}$. Based on the first criteria, we introduce a relational head as a learnable function to enforce the similarity between estimated $\hat{\mathcal{Z}}$ from the same trajectory, thus eliminating contexts-specified redundant information. However, only clustering $\hat{\mathcal{Z}}$ in the same trajectory cannot guarantee $\hat{\mathcal{Z}}$ is semantically meaningful. This is because different trajectories may be sampled from the same environment, and thus the factors $\hat{\mathcal{Z}}$ belonging to different trajectories can share the same or similar semantics. Based on the criteria (b), we propose an interventional prediction method to measure the similarity between estimated $\hat{\mathcal{Z}}$ from different trajectories, where estimated $\hat{Z}$ will be concatenated with all state-action pairs in a mini-batch to predict next states. According to the criteria (b) and the generalized dynamics function $\mathcal{F}: \mathcal{S} \times \mathcal{A} \times \mathcal{Z} = \mathcal{S}$, high similarity will be assigned into factors $\hat{\mathcal{Z}}$ that have similar next state predictions. By means of the proposed relational head, factors $\hat{\mathcal{Z}}$ across trajectories but with similar semantics can be clustered, and thus the estimated $\hat{\mathcal{Z}}$ can generalize on different trajectories and eliminate those contexts-specified and the single trajectory-specified spurious redundant information. In the experiments, we evaluate our method on a range of tasks in OpenAI gym \cite{brockman2016openai} and Mujoco \cite{todorov2012mujoco}, and the sufficient results show that the performance of our method exceeds the state-of-art model-based RL methods.
% two criteria, we propose a relational intervention approach to estimate unobserved environment-specified factors  $Z$ explicitly.
% and semantic meaningfully and improve the generalization ability of model-based RL. Firstly, we use an encoder to distil the unobserved task-specified factors $Z$  into a vector from transition segments of each task, and then the distilled vector $\hat{Z}$ is incorporated into the dynamics prediction model $f$ in the model-based RL methods, enabling the estimated $\hat{Z}$ can help $f$ generalize well on other tasks with unseen dynamics. Then taking advantage of the homogeneity of the $Z$ in a single trajectory, a relational head is used to discriminate whether the distilled factor vector relates to vectors from the same trajectory, which clusters the estimated $\hat{Z}$ from the same trajectory without modelling irrelevant dependencies, \emph{e.g.} context information. Lastly, we propose a interventional prediction module to make full use of inter-trajectory information in a mini-batch, making the learned task-specified factor  $\hat{Z}$ more semantically meaningful. This module infers the multiple-relations between task-specified factors $Z$ in different trajectories by measuring their similarities. Every estimated factor $\hat{z_i} \in \hat{Z}$  in a mini-batch will be used to predict the next state belong to other trajectories in this module, \emph{i.e.} interventional prediction. The high similarity will be assigned to those factors that have similar next state predictions over a mini-batch \emph{e.g.} two factors are from trajectories but belong to the same task. By means of relational head, we can cluster factors $\hat{Z}$ with similar semantics but in different trajectories in an unsupervised manner.
% In the experiments, we evaluate our method on a range of tasks in OpenAI gym \cite{brockman2016openai} and Mujoco \cite{todorov2012mujoco}, and the sufficient results show that the performance of our method exceeds the state-of-art model-based RL methods.


%\textbf{Contribution} (1) We propose a encoder based on the relational learning, enabling the 

% (distilled factors from the same trajectory) or not (with distilled factor from other trajectories). 

%of the distilled   and relational learning, the proposed encoder is trained to maximize the mutual information between trajectories and underlying confounder, and discard the useless information, \emph{e.g.} context information, thus disentangling meaningful confounder embedding from history trajectory.

%In the experiments, we combine the confounder embedding extracted from proposed contrastive confounder encoder into both model-based RL and model-free RL methods, and then evaluate them on a range of tasks in OpenAI gym \cite{brockman2016openai} and Mujoco \cite{todorov2012mujoco}. Sufficient experimental results show:
%\begin{enumerate}
%	\item Our contrastive confounder encoder shows superior generalization ability on unseen tasks with different transition functions, and the performance even exceed state-of-the-art RL methods.
%	\item Our contrastive confounder encoder shows higher sample-efficiency on model-based RL.
%	\item The visualization results
%\end{enumerate}
% the sights, scents, andsounds of baking, driven by a propose a confounder encoder to distill the confounder information that can potentially change the transition function.
%
%taking a tennis game as an example, when you 
%is so high that they need a large amount of data or interactions with the environment to optimize the agent's behaviour.  
% different opponents will hit back the tennis ball in different policies when facing the same incoming ball, and thus you need to 





==> methods.tex <==
\subsection{Overview} \label{sec:mot}
%We believe that s
\begin{figure*}[!htb]
%	\vspace{-1em}
%	\begin{center}
%		\includegraphics[height=2.5in]{figures/framework.pdf}
		
%		\label{img:over}
%		\vspace{-0.5em}
%	\end{center}
	\vspace{-1em}
	\subfloat{      
	\begin{minipage}[c]{1\linewidth}
		\centering
		\label{img:over}
		\includegraphics[scale=0.38]{figures/framework.pdf}
		%				             \includegraphics[width=1.2\textwidth]{MKDB_KDB_RMSE_ALL.pdf}
		%			\includegraphics[height=1.2in]{figures/training_aba.pdf}
	\end{minipage}
}
	\caption{{An overview of our Relational Intervention approach, where Relational Encoder, Prediction Head and Relational Head are three learnable functions, and the circles denote states (Ground-Truths are with {red boundary}, and estimated states are with black boundary), and the rectangles denote the estimated vectors. Specifically, $prediction\ Loss$ enables the estimated environmental-specified factor can help the Prediction head to predict the next states, and the $relation\ Loss$ aims to enforce the similarity between factors estimated from the same trajectory or environments. } }
	\vspace{-1em}
\end{figure*}
%
% The main intuition behind our approach is that there are other environment-specified factors $\mathcal{Z}$, in addition to the state $\mathcal{S}$ and action $\mathcal{A}$, can affect the output of dynamics function $f: \mathcal{S}\ \times  \mathcal{A} \rightarrow  \mathcal{S}$.  
%Seeing \textcolor{red}{Figure}    as an example, the goal of the Pendulum task is to swing up a rigid body and keep it in the upright position. The state given in this task is the angle and the angular velocity of the rigid body from the upright position, and the action is the effort enforced on the rigid. Obviously, the given state still satisfies the nature of MDP, but there are unobserved environment-specified factors that can affect the dynamics function of rigids, such as the length and mass of rigids.  If we swing up other rigids with different lengths, the learned dynamics model $F$ will fail to provide accurate predictions because of the change of rigid's length, and causes the performance decline of model-based methods. 
%We can see other examples about that $\mathcal{Z}$ can potentially change the dynamics functions of MDPs, \emph{e.g.} a trained robot walks on grounds with different frictional resistances,  boxing with opponents who use different strategies or with different force classes. 

As analyzed in Section \ref{sec:intro}, we can incorporate the environment-specified factors $Z\in \mathcal{Z}$ into the dynamics prediction process to generalize the dynamic functions on different environments, \emph{i.e.} extending the dynamics function from $f:\mathcal{S}\ \times  \mathcal{A} \rightarrow  \mathcal{S}$\ to\ $f:\mathcal{S}\ \times  \mathcal{A}\ \times\ \mathcal{Z} \rightarrow  \mathcal{S}$. Because $Z$ is the same within an environment, we expect estimated $\hat{Z}$s from the same environment are similar while those from different environments are dissimilar. Therefore, $f$ models the commonalities of the transition dynamics in different environments and $Z$ models the differences.
In the supervised dynamics generalization setting, where the environment id is given, one can easily learn $Z$ by using metric losses, \emph{e.g.}, CPC \citep{oord2018representation} and relation loss \citep{patacchiola2020self} to enforce that the estimated $\hat{Z}$s are similar in the same environment and dissimilar in different environments. However, since the environment label is unavailable in the unsupervised setting, we have to simultaneously learn $Z$ and discover the cluster structures. To this end, we propose an intervention module to measure the similarities between each pair of $\hat{z}_i$ and $\hat{z}_j$ as the probability of them belonging to the same environment. Furthermore, we then introduce a
relational head to aggregate  $\hat{Z}$s with high probability using relation loss. By simultaneously updating the dynamics prediction and the relation loss, we can cluster $\hat{Z}$s from the same environment, and learn an augmented dynamics prediction model $\hat{{f}}$. Next, we will give details about our relational intervention approach.
%Utilizing the invairiance of $Z$ within an single environment, we can directly clusrer $Z$ according to their environment label and learn it with the dynamics prediction. Unfortunately, the environment label is unavailable in the unsupervised setting, and because the transition
% However, because transition segments contain much Therefore, the estimated  $\hat{{Z}}$ inevitable contains  transition segments-specified and trajectory-specified redundant information. %  limiting the generalization ability of the dynamics prediction model.
% Therefore, estimating a semantically meaningful $\mathcal{Z}$  without irrelevant dependencies is the key step to learn generalized dynamics function.
%As such, the change of dynamics functions $\mathcal{F}$ across environments can be modelled as the change of factors $\mathcal{Z}$. 
% These factors $\mathcal{C}$ remain same in one MDP, but may vary in different MDPs.
% Here we can call these underlying factors $\mathcal{C}$ as a confounder in RL, because it influences the state and action at the same time by changing the transition function.
%To estimate ${Z}$ which reflects the dynamics change, we summarize two criteria that true ${Z}$ should meet, but other redundant information should not:  
%\begin{enumerate}[a.]
%	\item The factors $\hat{{Z}}$ estimated from one trajectory should be the same.  
%
%	\item Given two semantically similar estimated $\hat{{Z}}$, the output distributions of dynamics function should be similar if  conditioned the same state-action pairs.  
%\end{enumerate}
%Criterion (a) is sensible because a trajectory is surely sampled from one environment.  According to the extended generalized dynamics function $f: \mathcal{S} \times \mathcal{A} \times \mathcal{Z} = \mathcal{S}$, if the state and action remain the same, ${Z}$ is the only factor can change the output distribution of $f$, and thus the criteria (b) is well established.  Based on these two criteria, we propose a \textit{Relational Intervention} approach to distill environment-specified ${Z}$ and eliminate  transition segments-specified and trajectory-specified redundant information. The overall framework of our approach is shown Figure \ref{img:over}. We first use a relational encoder to estimate $\hat{{Z}}$  from the sampled  transition segments  \citep{seo2020trajectory,lee2020context,rakelly2019efficient,zhou2019environment}. Then,  we use a relational head as a learnable function to identify whether two estimated $\hat{{Z}}$ are from the same trajectory or not and enforce the similarity into factors $\hat{{Z}}$ from the same trajectory to meet the criteria (a). Lastly, by means of intervention operation, we calculate the distribution of next states conditioned on the same state-action pairs and different $\hat{{Z}}$ in a mini-batch. The high similarity will be assigned into the factors $\hat{{Z}}$ with small distance between their output distributions. Similar as before, the proposed relational head can impose similarity on factors $\hat{{Z}}$ with high similarity, and thus the $\hat{{Z}}$ can generalize on different trajectories, eliminating the  transition segments and single trajectory specified redundant information. 
% cluster $Z$ within each trajectory by a binary relational reasoning.  However, different trajectories may belong to the same environment, and thus share the same environment-specified factor $Z$. We propose a counterfactual prediction module to cluster $Z$ that are semantically similar without knowing the environment id of trajectory.
% In this paper, we propose a module called \textit{Counterfactual Relational Encoder} to distill the task-specified factors $Z$ by learning the relationship between different trajectories using relational network. The overview of our approach is as Figure \ref{img:over} shown, we firstly build a relational encoder to extract task-specified factor $z^i$ from a trajectory segments $\tau^i_{t-k,t} = \{(s_{t-k},a_{t-k}),...,(s_t,a_t)\}$, and then the estimated $z_i$ is i.  
% can However, since different trajectories may belong to the same MDP, simply distinguishing different trajectories may misclassify the trajectories with same factors $Z$. In addition, the similarity  between factors $Z$ are different,  \emph{e.g.} the trajectory of rigids with the length 0.8 are more similar with those length 1 than rigids with length 2.  While the vanilla relational network cannot reflect  how similar of different taks-relevant factors $Z$ . Therefore, we propose a counterfactual prediction similarity to denote the how similar of 
% is unobservable, how to estimate it from trajectories is a challenge problem
%Next,  we will give details about proposed Relational Intervention approach.


%t generalization of RL methods over a collection of MDPs $\{\mathcal{M}_i\}_{i=0}^{N}$ that Normally, standard RL methods trained in one MDP $\mathcal{M}_i$ cannot generalize well 
%a key step is to find the underlying factors $\mathcal{C}$ that can change the transition functions for each task. 
\subsection{Relational Context Encoder} \label{sec:relation}
To learn the environment-specified factor $Z$ of each environment, we firstly introduce a relational encoder $g$ parameterized by $\phi$. Similar to previous methods \citep{nagabandi2018learning,rakelly2019efficient,zhou2019environment,lee2020context,seo2020trajectory}, we use the past transition segments $\tau_{t-k:t-1} = \{(s_{t-k},a_{t-k}),...,(s_{t-1},a_{t-1})\}$ as the input of  $g$ to estimate its corresponding $\hat{z}_{t-k:t-1}$:
$$\hat{z}_{t-k:t-1}=g(\tau^{i}_{t-k:t-1};\phi).$$
After obtaining environment-specified $\hat{z}_{t-k:t-1}$ at timestep $t$, we incorporate it into the dynamics prediction model $\hat{f}$ to improve its generalization  ability on different dynamics by optimizing the objective function following  \citep{lee2020context,seo2020trajectory,janner2019trust}:
\begin{equation}
%	\hat{z}^i_{i-k,t-1} = g(\tau^i_{t-k,t-1};\phi)
%	\label{eq:context}
	\mathcal{L}^{pred}_{\theta,\phi}\ =\  -\frac{1}{N} \sum_{i=1}^{N}\  \log \  \hat{f}(s_{t+1}^{i}|s_t^{i},a_t^{i},g(\tau^{i}_{t-k:t-1};\phi);\theta),
	\label{eq:prediction}
\end{equation}
where $k$ is the length of transition segments, $t$ is the current timestep and $N$ is the sample size. In practice, we sub-sample a mini-batch of data from the whole dataset to estimate (\ref{eq:prediction}) and use stochastic gradient descent to update the model parameters. 
%Specifically, $\hat{f}$ is modelled as a gaussian function, limited b
% Here we also use the auxiliary prediction loss likes \citep{lee2020context} to predict the backforward and future states.
%The loss \ref{eq:prediction} enables the estimated $\hat{z}^i_{i-k,t-1}$ to help $f$ generalize well on environments with dynamics changes. 

However, as analyzed in Section \ref{sec:mot}, the vanilla prediction error  (\ref{eq:prediction}) is not sufficient to capture environment-specified $Z$ of each environment, and even introduce redundant information into it.  In order to eliminate the redundant information within transition segments and preserve the trajectory invariant information, we introduce a relational head \citep{patacchiola2020self} as a learnable function $h$ to pull factors $\hat{Z}$ from the same trajectory together and push away those from different trajectories. Concretely, the estimated $\hat{z}^{i}_{t-k:t-1}$ in a mini-batch will be firstly aggregated as pairs, \emph{e.g.} concatenate two factors as $[\hat{z}^{i}, \hat{z}^{j}]$, and the pairs having two factors from the same trajectory are seen as positives, and vice versa. Then the relational head $h$ parameterized by $\varphi$ takes a pair of aggregated factors as input to quantify the similarity of given two factors and returns a similarity score $\hat{y}$.  To increase the similarity score $\hat{y}$ of positive pairs and decrease those negatives, we minimize the following objective:
\begin{equation}
	%	\hat{z}^i_{i-k,t-1} = g(\tau^i_{t-k,t-1};\phi)
	%	\label{eq:context}
	\mathcal{L}^{relation}_{\varphi,\phi}\ =\  -\frac{1}{N(N-1)} \sum_{i=1}^{N} \sum_{j=1}^{N}\Big [ \ y^{i,j} \cdot \log \ h([\hat{z}^i,\hat{z}^j];\varphi) + (1-y^{i,j})  \cdot  \log \ (1 - h([\hat{z}^i,\hat{z}^j];\varphi)) \Big ],
%	 f(s_{t+1}^{i,j}|s_t^{i,j},a_t^{i,j},g(\tau^{i,j}_{t-k:t-1};\phi);\theta)
	\label{eq:relation}
\end{equation}
where $y^{i,j}$ = 1 stands for positive pairs, and $y^{i,j}$ = 0 stands for negatives.
Because the positive pairs have two factors belonging to the same trajectory, optimizing (2) can increase the similarity of $\hat{{Z}}$s
estimated from the same trajectory, and push away those factors estimated from different trajectories in their semantical space. Therefore, by optimizing (\ref{eq:relation}), the information that is invariant within a trajectory will be encoded into $\hat{Z}$ and the redundant information in transition segments will be reduced. (\ref{eq:relation}) can also be interpreted from the perspective of mutual information, if we regard the $\hat{{Z}}$s from the same trajectory as the positive pairs, optimizing (\ref{eq:relation}) can be seen as maximizing the mutual information between $\hat{{Z}}$s from the same trajectory (Please refer to \citep{tsai2020neural} and Appendix \ref{sec:mi}), and thus preserve the invariant information with the same trajectory. 
However, estimating trajectory invariant information is insufficient because the estimated $\hat{{Z}}$s in the same environment will also be pushed away, which may undermine the cluster compactness for estimated $\hat{{Z}}$s.
%Following the setting of \citep{sung2018learning,hu2018relation,patacchiola2020self}, the aggregation method in our paper is concatenation

% A key step to improve dynamics generalization of RL methods  is to find the underlying factors $\mathcal{C}$ that can change the transition functions.
%Because $\mathcal{C}$ is unobserved,  and thus we need to learn it from the trajectories $\mathcal{X}:  X^{tr}_i=\{s_0,a_0,s_1,a_1 ... s_T, a_T\}^{tr}_i$ of training tasks  $\{\mathcal{M}_i^{tr}\}_{i=0}^{K}$ with different $\mathcal{C}_i^{tr}$. 
%However, the trajectory contains  redundant information which is unrelated to $\mathcal{C}$, \emph{e.g.} the state and action information. To discard these information and encode confounder $\mathcal{C}$ into a compact vector, we maximize the mutual information between $\mathcal{X}$ and $\mathcal{C}$: \\
%\begin{equation}
%	I(X,C) =  
%\end{equation}

%According to the analysis in the \ref{sec:mot}, the transition function can be written as, $P(s_{t+1}|s_t,a_t,c)$, and trajectories in the task $i$ can be formulized as:
%Then we combine it into dynamics prediction model in model-based RL and policy network in model-free RL to 
\begin{figure}[!htb]
		\vspace{-0.5em}
		\centering
%	\begin{center}
%		\includegraphics[height=1.8in]{figures/counterfactual.pdf}
		
%		\label{conter}
%		\vspace{-0.5em}
%	\end{center}
%	\subfloat[]{      
%	\begin{minipage}[c]{.33\linewidth}
%		\centering
%		\includegraphics[scale=0.55]{figures/causal.pdf} 
%			\label{fig:causal} 
%	\end{minipage}
%}
%	\hspace{0.1in}
%\subfloat[]{      \begin{minipage}[c]{.66\linewidth}

\includegraphics[scale=0.43]{figures/intervention.pdf}

%\end{minipage}}
%	\hspace{1in}
%\subfloat[]{      \begin{minipage}[c]{.23\linewidth}
%\includegraphics[scale=0.23]{figures/pca_pendulum_tmcl.pdf}\end{minipage}}
%\hspace{1in}
%\subfloat[]{      \begin{minipage}[c]{.23\linewidth}
%\includegraphics[scale=0.23]{figures/pca_pendulum_our.pdf}\end{minipage}}
		%				             \includegraphics[width=1.2\textwidth]{MKDB_KDB_RMSE_ALL.pdf}
		%			\includegraphics[height=1.2in]{figures/training_aba.pdf}
%	\end{minipage}


	\caption{(a) The illustration of causal graph, and the red line denotes the direct causal effect from $Z$ to $S_{t+1}$. (b) The illustration of estimating the controlled causal effect.}
	\label{fig:inter}
		\vspace{-1.em}
\end{figure}
%\begin{algorithm}
%	\caption{Relational Intervention Training Approach}
%	\label{alg:A}
%	\begin{algorithmic}
%		\State {Initialize parameters of relational encoder $\phi$, dynamics prediction model $\theta$ and relational head $\varphi$}
%		\State  {Initialize dataset $\mathcal{B} \gets \emptyset$} 
%		\For{Each Iteration}
%		\State  sample environments $\mathcal{M}^i$  from training environments      $\{\mathcal{M}_i^{tr}\}_{i=0}^{K}$       \Comment{Collecting Data}
%		\For{$T=1$ to TaskHorizon}
%		%		\STATE $//$ Collecti
%		\State Get the estimation of the environment-specified factor  $\hat{z}_{t-k:t-1}^i=g(\tau_{t-k:t-1}^i;\phi)$
%		\State{Collect {($s_t,a_t,s_{t+1},r_t,\tau_{t-k:t-1}^i$)} from  $\mathcal{M}^i $ with dynamics prediction model $\theta$ }
%		\State{Update $\mathcal{B} \gets  \mathcal{B} \cup (s_t,a_t,s_{t+1},r_t,\tau_{t-k:t-1}^i)$}
%		\EndFor
%		\For{Each Dynamics Training Iteration} \Comment{Update  $\phi$,$\theta$  and $\varphi$}
%		\For{$k=1$ to K } 
%		\State Sample data $\tau_{t-k:t-1}^{i,b,P}$ , $\tau_{t:M}^{i,b,K}$ with batch size B,from $\mathcal{B}$
%		\State Get the estimation of the environment-specified factor  $\hat{z}_{t-k:t-1}^{i,B,,P}=g(\tau_{t-k:t-1}^{i,B,P};\phi)$
%		\State Compute the total loss \State$\mathcal{L}^{tot}$=$\mathcal{L}^{pred}_{\phi,\theta}(\tau_{t:M}^{i,B,,K},\hat{z}_{t-k:t-1}^{i,B,,P})+\mathcal{L}^{i-relation}_{\phi,\varphi}(\hat{z}_{t-k:t-1}^{i,B,,P})+\mathcal{L}^{dist}_{\phi,\theta}(\tau_{t:M}^{i,B,K},\hat{z}_{t-k:t-1}^{i,B,P})$
%		\State Update $\theta \ ,\ \phi \ ,\ \varphi  \gets \nabla_{\theta  ,\phi \,\varphi } \frac{1}{B}\mathcal{L}^{tot}$
%		\EndFor
%		\EndFor
%		\EndFor
%	\end{algorithmic}
%\end{algorithm}
\vspace{-0.5em}
\subsection{Interventional  Prediction}
 Because the environment id of a trajectory is unknown, we cannot directly optimize relational loss (\ref{eq:relation}) to cluster $\hat{{Z}}$ within an environment. We propose an interventional prediction method to find the trajectories belonging to the same environment. Here we formalize the dynamics prediction model using a graphical causal model, and the causal graph is illustrated as Figure \ref{fig:inter} (a), where the next state $S_{t+1}$ is caused by the current state $S_{t}$, action $A_{t}$ and $\hat{Z}$, and the dynamics prediction model $f $ represents the causal mechanism between them. Because $Z$ from the same environment should have the same influence on the states, and thus they should have the same causal effect on the next state $S_{t+1}$ if given $S_t$ and $A_t$ under the causal framework. As such, we can find estimated $\hat{{Z}}$ belonging to the same environment by measuring the similarity of their causal effect on $S_{t+1}$. As Figure \ref{fig:inter} (a) shows, there are multiple paths from $Z$ to $S_{t+1}$ and we roughly categorize them into two categories. The first category is the direct path between $Z$ and $S_{t+1}$ ( shown as read in Figure \ref{fig:inter}). The second category contains all the indirect paths where $Z$ influences $S_{t+1}$ via previous states and actions.
%  \begin{align}
%  	%	\hat{z}^i_{i-k,t-1} = g(\tau^i_{t-k,t-1};\phi)
%  	%	\label{eq:context}
%  	P(S_{t+1}|Z) =  P(S_{t+1}|Z,S_t,A_t)P(A_t|Z,S_t)P(S_t|Z, pa(S_t)_{/Z})P(Z)P(pa(S_t)_{/Z})
%  	\label{eq:prob}
%  \end{align}
  However, because the mediator in other paths \emph{e.g.} $S_t$, $A_t$, may amplify or reduce the causal effect of $Z$, we only consider the direct path from $Z$ to the next state(denote by the red line at Figure \ref{fig:inter} (a)), which means that we need to block all paths with meditors from $\hat{{Z}}$ to $S_{t+1}$. By means of do-calculus \citep{pearl2000causality}, we can estimate the direct causal effect of changing $Z=\hat{z}^j$ to $Z=\hat{z}^k$ on $S_{t+1}$ through calculating the controlled direct effect (CDE) \citep{pearl2013direct} by intervening mediators and $\hat{{Z}}$ :
  \small
\begin{align}
	\small
	%	\hat{z}^i_{i-k,t-1} = g(\tau^i_{t-k,t-1};\phi)
	%	\label{eq:context}
 CDE_{\hat{z}^j,\hat{z}^k}(s_t,a_t)=&\mathbb{E}[S_{t+1}|do(S_t =s_t,A_t=a_t),do(Z=\hat{z}^j)] 
	- \mathbb{E}[S_{t+1}|do(S_t =s_t,A_t=a_t),do(Z=\hat{z}^k)] \\
	=&\mathbb{E}[S_{t+1}|S_t =s_t,A_t=a_t,Z=\hat{z}^j]  
	- \mathbb{E}[S_{t+1}|S_t =s_t,A_t=a_t,Z=\hat{z}^k],
	\label{eq:cde}
\end{align}
\normalsize
where $do$ is the do-calculus \citep{pearl2000causality}. There is no arrow entering $\hat{{Z}}$, so the do operator on $\hat{{Z}}$ can be removed. Also, since there is no confounder between the mediators $(S_t, A_t)$ and $S_{t+1}$, so we can remove the do operator of them as well, and the equation become as (\ref{eq:cde}).
Because the direct causal effects may differ for different values of $S_t$ and $A_t$, we should sample $S_t$ and $A_t$ independently of $Z$, \emph{i.e.} sampling $S_t$ and $A_t$ \citep{pearl2016causal} uniformly to get the average controlled direct causal effect from $\hat{{Z}}$ to $S_{t+1}$. However, if we use the uniformly generated $S_t$ and $A_t$, the sampled distribution may differ from the training distribution, resulting in inaccurate the next state prediction. As such, we directly sample $S_t$ and $A_t$ from the observational data. For the convenience of optimization, we only use a mini-batch of $S_t$ and $A_t$ pairs $(s_t^i,a_t^i)$, and concatenate them with $\hat{z}^j$ and $\hat{z}^k$ to calculate the average controlled direct effect under $\hat{f}$:
% \small
 \begin{align}
 	%	\hat{z}^i_{i-k,t-1} = g(\tau^i_{t-k,t-1};\phi)
 	%	\label{eq:context}
%  	ACDE_{\hat{z}^j,\hat{z}^k}= \frac{1}{N}\sum_{i=1}^{N}\lvert\mathbb{E}[S_{t+1}|S_t =s_t^i,A_t=a_t^i,Z=\hat{z}^j] 
%  	- \mathbb{E}[S_{t+1}|S_t =s_t^i,A_t=a_t^i,Z=\hat{z}^k]\rvert
 	 	ACDE_{\hat{z}^j,\hat{z}^k}= \frac{1}{N}\sum_{i=1}^{N}\lvert CDE_{\hat{z}^j,\hat{z}^k}(s_t^i,a_t^i)\rvert,
 	\label{eq:fcde}
 \end{align}
%\normalsize
%By the mean of do-calculus \citep{pearl2000causality} in causal inference, we can solely estimate the causal effect of a certain environmental-specified factor $\hat{z}$ on the predict distribution in a mini-batch, and thus eliminate the perturbation of the dynamic prediction model from the state-action pairs.
%\begin{equation}
%	%	\hat{z}^i_{i-k,t-1} = g(\tau^i_{t-k,t-1};\phi)
%	%	\label{eq:context}
%	P_f(S_{t+1}|do(Z=\hat{z}))\ = \sum_{i=1}^{N} P_{\hat{f}}(S_{t+1}|S_t = s_{t}^i, A_t = a_{t}^i, do(Z =\hat{z}))
%		\label{eq:do}
%\end{equation}
where $N$ is the batch size, $j$ and $k$ are the id of $\hat{{Z}}$ estimated from two transition segments.
%According to the criteria (b), $\hat{z}$ with similar semantics should have similar output distribution if conditioned on the same state action pairs. As such, we can extent the standard do-calculus as follows to measure the difference between two different interventions $\hat{z}^j$ and $\hat{z}^k$ by measuring the distance between their dynamics prediction distribution:
%\begin{align}
% 	%	\hat{z}^i_{i-k,t-1} = g(\tau^i_{t-k,t-1};\phi)
% 	%	\label{eq:context}
% d^{j,k}=  \frac{1}{N}	\sum_{i=1}^{N} \mathcal{W}_1 \Big [ P_{\hat{f}}(S_{t+1}|S_t = s_{t}^i, A_t = a_{t}^i, do(Z = \hat{z}^j)), P_{\hat{f}}(S_{t+1}|S_t = s_{t}^i, A_t = a_{t}^i, do(Z = \hat{z}^k))\Big ]
% 	\label{eq:two-do}
%\end{align}
%where $N$ is the batch size, $j$ and $k$ are the id of factors estimated from two transition segments, and we use the $\mathcal{W}_1$  1-Wasserstein distance \citep{villani2009optimal} as the distance metric to capture the difference between two output distribution resulting from two interventions. 
 Specifically, because the factors $\hat{z}$ estimated from the same trajectory should be the same, and thus we minimize their controlled direct effect \ref{eq:fcde} as $\mathcal{L}^{dist}$ between them in the optimization process.
Now we can use the calculated $ACDE_{\hat{z}^j,\hat{z}^k}$ as the semantic distance $d^{j,k}$ between estimated $\hat{z}^i$ and $\hat{z}^j$, and thus we can aggregate factors ${\hat{Z}}$ estimated from similar trajectories by the proposed relational head $h$. As such, we apply a transformation to convert distance metric $d^{j,k}$ to a similarity metric $w \in (0,1]$, which  is $w^{j,k} = exp(\frac{-d^{j,k}}{\beta})$, where $\beta$ is a factor controlling the sensitivity of the distance metric. Specifically, because the scale and size of state varies in different tasks, \emph{e.g.} 3 dims in Pendulum but 20 dims in Half-Cheetah, the optimal $\beta$ may vary in different task. As such, we apply the  normalization in the distance metric $d$, \emph{i.e.}, normalize $d$ with batch variance, to convert it as a relative distance within a single task, thus making the optimal $\beta$ stable in different tasks. Then we can directly aggregate similar trajectories by extending the loss function (\ref{eq:relation}) as follows:
% \begin{equation}
\begin{align}
	%	\hat{z}^i_{i-k,t-1} = g(\tau^i_{t-k,t-1};\phi)
	%	\label{eq:context}
	\mathcal{L}^{i-relation}_{\varphi,\phi}\ =\ &  -\frac{1}{N(N-1)} \sum_{i=1}^{N} \sum_{j=1}^{N}\Big [ \ [y^{i,j} + (1-y^{i,j})\cdot w^{i,j}] \cdot \log \ h([\hat{z}^i,\hat{z}^j];\varphi) \nonumber \\
	&+ (1-y^{i,j}) \cdot (1-w^{i,j})  \cdot  \log \ (1 - h([\hat{z}^i,\hat{z}^j];\varphi)) \Big ],
	%	 f(s_{t+1}^{i,j}|s_t^{i,j},a_t^{i,j},g(\tau^{i,j}_{t-k:t-1};\phi);\theta)
	\label{eq:i-relation}
\end{align}
% \end{equation}
where the first term indicates that the factors from the different trajectories can be aggregated with the similarity weight $w$ and 1 those from the same trajectory, and the second term means that factors from different trajectories should be pushed with each other with weight $1-w$. 
Similar to the analysis in section 3.3, optimizing the loss function (6) can increase the similarity between $\hat{{Z}}$ with weight $w$, and push away from them with the weight $1-w$. Because $\hat{{Z}}$s estimated from the same environment have similar effects, these factors will be assigned with high similarities  (estimated by the intervention operation of our paper).
By simultaneously updating the prediction loss (\ref{eq:prediction}) and intervention relation loss \ref{eq:i-relation}, estimated $\hat{{Z}}$s within the same environment will be aggregated, and the learned dynamics function $\hat{{f}}$ can learn the modals of transition dynamics according to the $\hat{{Z}}$ in different clusters.
The training procedure of our approach can refer to Algorithm process in Appendix \ref{sec:alg}.



%a model the change of transition functions across different tasks and enable RL methods robust to the transition shift , we introduce a confounder variable to model the variantion of 

==> preliminaries.tex <==
\subsection{Problem Setup}
The standard reinforcement learning task can be formalized as a Markov  decision  process  (MDP)
 $\mathcal{M}\ =\ (\mathcal{S}, \mathcal{A}, r, p, \gamma, \rho_0)$ over discrete time \citep{puterman2014markov, sutton2018reinforcement}, where $\mathcal{S}$, $\mathcal{A}$,  $\gamma \in (0,1]$, $\rho_0$  are  state space,  action space,  the reward discount factor, and the initial state distribution, respectively. The reward function $r:\ \mathcal{S}\ \times  \mathcal{A} \rightarrow \mathbb{R}$ specifies the reward at each timestep $t$ given  $s_t$ and $a_t$, and transition dynamics $p(s_{t+1}|s_t,a_t)$ gives the next state distribution conditioned on the current state $s_t$ and action $a_t$.  The goal of RL is to learn a policy $\pi( \cdot |s)$ mapping from state $s \in \mathcal{S}$ over the action distribution to maximize the cumulative expected return over timesteps $\mathbb{E}_{s_t\in \mathcal{S}, a_t\in \mathcal{A}}[\sum_{t=0}^\infty \gamma^t\ r(s_t,a_t)]$. In model-based RL, a model ${f}$ is used to approximate the transition dynamics $p$, and then ${f}$ can provide training data to train policy $\pi$ or predict the future sequences for planning. Benefiting from data provided by learned dynamics model ${f}$, model-based RL has higher data efficiency and better planing ability compared with model-free RL.

Here we consider the unsupervised \textit{dynamics generalization} problem in model-based RL, where we are given K training MDPs $\{\mathcal{M}_i^{tr}\}_{i=1}^{K}$ and L test MDPs $\{\mathcal{M}_j^{te}\}_{j=1}^{L}$ that have the same state and action space but disjoint dynamics functions, and we randomly sample several MDPs from training MDPs in each training iteration. We assume that all these MDPs have a finite number of dynamics functions, meaning that the MDPs can be categorized into a finite number of environments and the MDPs in each environment share the same dynamics function but the environment id of MDPs is unavailable in the training process. In the context of model-based RL, how to learn a generalized dynamics model ${f}$ is the key challenge to solve unsupervised \textit{dynamics generalization} problem.


==> related.tex <==
%\section{Related Work}
%\textbf{Model-Based Reinforcement Learning}  \quad Model-based Reinforcement learning (MBRL) enjoys the benefit of high data efficiency by explicitly learning a predictive model to approximate the dynamics function of environments. The learned predictive model can generate samples as priors for training policy efficiently \cite{du2019task,whitney2019dynamics} or planning before choosing actions in the inference \cite{atkeson1997comparison,lenz2015deepmpc,tassa2012synthesis}. The performance of MBRL highly relies on the prediction accuracy of the dynamics predictive model. As such, numerous methods are proposed to improve the predictive model's accuracy, \emph{e.g.} ensemble methods \cite{chua2018deep}, latent dynamics model \cite{hafner2019learning,hafner2019dream,schrittwieser2020mastering}. However, current predictive methods still hard to generalize well on unseen dynamics.\\
\textbf{Dynamics Generalization in MBRL} \quad  Several meta-learning-based MBRL methods are proposed \cite{nagabandi2018learning,nagabandi2018deep,saemundsson2018meta,huang2021adarl} to adapt the MBRL into environments with unseen dynamics by updating model parameters via a small number of gradient updates \cite{finn2017model} or hidden representations of a recurrent model \cite{doshi2016hidden}, and then \cite{wang2021model} proposes a graph-structured model to
improve dynamics forecasting. {\cite{ball2021augmented} focuses on the offline setting and proposes an augmented model method to achieve zero-shot generalization.}  \cite{lee2020context,seo2020trajectory} try to learn a generalized dynamics model by incorporating context information or clustering dynamics implicitly using multi-choice learning, aiming to adapt any dynamics without training. However, how to explicitly learn the meaningful dynamics change information remains a big challenge.
%\cite{Many methods }
\\
\textbf{Relational Learning}  \quad  Reasoning relations between different entities is an important way to build knowledge of this world for intelligent agents \cite{kemp2008discovery}. In the past decades,  relational paradigm have been applied to a wide range of deep learning-based application, \emph{e.g.}, reinforcement learning \cite{zambaldi2018deep}, question-answer \cite{santoro2017simple,raposo2017discovering}, graph neural network \cite{battaglia2018relational}, sequential streams \cite{santoro2018relational}, few-shot learning \cite{sung2018learning}, object detection \cite{hu2018relation} and self-supervised learning \cite{patacchiola2020self}. Different from previous methods that perform binary relational reasoning on entities, our method can also perform multiplies relations between entities through the learned similarity of entities, and thus can learn more compact and meaningful entity representation.  \\
\textbf{Causality in Reinforcement Learning} \quad Many works focus on the intersection area of reinforcement learning and causal inference. For example, some works aims to alleviate the causal confusion problem in the imitation learning \citep{de2019causal,zhang2020causal,kumor2021sequential}, batch learning \citep{bannon2020causality},
and partial observability settings \citep{forney2017counterfactual,kallus2018confounding,zhang2019learning,lu2018deconfounding} in the online environment \citep{lyle2021resolving, zhang2018fairness}, \citep{wang2020provably} also try to apply causal inference in the offline setting, where the observational data is always confounded. \cite{lee2018structural,bareinboim2015bandits,lattimore2016causal,mozifian2020intervention,volodin2020resolving} also explore how to design an optimal intervention policy in bandits or RL settings. In addition, \citep{zhang2020invariant, zhang2020learning} improve the generalization ability of state
abstraction. Different from these methods, we focus on the setting of unsupervised dynamics generalization, and measure the direct causal effect \citep{pearl2013direct} between $\hat{{Z}}$ and the next state to estimate the probability of them belonging to the same environment.



